Redrock: Spectroscopic Classification and Redshift Fitting for the Dark Energy Spectroscopic Instrument

Redrock is a software package for spectroscopic classification and redshift fitting, designed to use the full information from spectroperfectionism outputs: flux-calibrated spectra, uncorrelated errors, and a per-spectrum resolution matrix encoding the non-Gaussian wavelength-dependent spectral line-spread function. Redrock was originally developed for the Dark Energy Spectroscopic Instrument (DESI), but the Extended Baryon Oscillation Spectroscopic Survey (eBOSS) also used Redrock as their primary galaxy redshift fitter prior to DESI. This paper presents the algorithmic details of Redrock and its performance on DESI data. On spectra from DESI DR2, Redrock achieves a redshift recovery rate of approximately 98% for the Bright Galaxy Survey (BGS) and Luminous Red Galaxies (LRG), 95.9% for Emission Line Galaxies (ELG), and 92.6% for quasars (QSO), and it delivers unbiased stellar radial velocities with a precision of roughly 5 km/s.

==> table-emlines.tex <==
\startlongtable
\begin{deluxetable}{ccc}
\tabletypesize{\footnotesize}
\tablecaption{Emission Lines\label{tab:emlines}}
\tablewidth{0pt}
\tablehead{
\colhead{Recombination} &
\colhead{Vacuum Wavelength} &
\colhead{Relative} \\
\colhead{Line} &
\colhead{(\AA)} &
\colhead{Flux}
}
\startdata
%\cutinhead{Recombination Lines}
  Ly$\alpha$ & 1215.670 &    23.54656 \\
   H$\alpha$ & 6564.613 &    2.863158 \\
    H$\beta$ & 4862.683 &    1.000000 \\
   H$\gamma$ & 4341.684 &   0.4683401 \\
   H$\delta$ & 4102.892 &   0.2589474 \\
 H$\epsilon$ & 3971.195 &   0.1590283 \\
       H6 & 3890.151 &   0.1050202 \\
       H7 & 3836.472 &  0.07312550 \\
       H8 & 3798.976 &  0.05302830 \\
       H9 & 3771.701 &  0.03971660 \\
      H10 & 3751.217 &  0.03053440 \\
      H11 & 3735.430 &  0.02399190 \\
      H12 & 3722.997 &  0.01920650 \\
      H13 & 3713.027 &  0.01561130 \\
      H14 & 3704.906 &  0.01286640 \\
      H15 & 3698.204 &  0.01073680 \\
      H16 & 3692.605 & 0.009052600 \\
  Pa$\alpha$ & 18756.13 &   0.3386235 \\
   Pa$\beta$ & 12821.59 &   0.1632389 \\
  Pa$\gamma$ & 10941.09 &  0.09044530 \\
  Pa$\delta$ & 10052.13 &  0.05545750 \\
Pa$\epsilon$ & 9548.591 &  0.03656680 \\
      Pa9 & 9231.547 &  0.02543320 \\
     Pa10 & 9017.385 &  0.01842910 \\
     Pa11 & 8865.217 &  0.01378950 \\
      P12 & 8752.876 &  0.01059920 \\
  Br$\alpha$ & 40522.62 &  0.08021050 \\
   Br$\beta$ & 26258.67 &  0.04546560 \\
  Br$\gamma$ & 21661.20 &  0.02781380 \\
  Br$\delta$ & 19450.87 &  0.01825910 \\
{\ion{He}{1}}~$\lambda3188$ & 3188.662 &  0.04076080  \\
{\ion{He}{1}}~$\lambda3389$ & 3889.752 &   0.1027011  \\
{\ion{He}{1}}~$\lambda3965$ & 3965.852 &  0.01022650  \\
{\ion{He}{1}}~$\lambda4026$ & 4027.348 &  0.02115760  \\
{\ion{He}{1}}~$\lambda4471$ & 4472.755 &  0.04445050  \\
{\ion{He}{1}}~$\lambda4922$ & 4923.304 &  0.01199870  \\
{\ion{He}{1}}~$\lambda5016$ & 5017.079 &  0.02568980  \\
{\ion{He}{1}}~$\lambda5876$ & 5877.299 &   0.1186800  \\
{\ion{He}{1}}~$\lambda6678$ & 6679.994 &  0.03360660  \\
{\ion{He}{1}}~$\lambda7065$ & 7067.198 &  0.02173860  \\
{\ion{He}{1}}~$\lambda10830$ & 10833.22 &   0.2404832  \\
%{[\ion{O}{3}]}~$\lambda5007$   & 5008.239  & 2.8875  \\
%{[\ion{O}{3}]}~$\lambda4959$   & 4960.295  & 1.0     \\
% {[\ion{N}{2}]}~$\lambda6584$  & 6585.277  & 2.93579 \\
% {[\ion{N}{2}]}~$\lambda6548$  & 6549.852  & 1.0     \\
% {[\ion{S}{2}]}~$\lambda6716$  & 6718.294  & 1.3     \\
% {[\ion{S}{2}]}~$\lambda6731$  & 6732.673  & 1.0     \\
% {[\ion{O}{2}]}~$\lambda3726$  & 3727.092  & 0.73    \\
% {[\ion{O}{2}]}~$\lambda3729$  & 3729.874  & 1.0     \\
% {[\ion{O}{1}]}~$\lambda6300$  & 6302.046  & 3.03502 \\
% {[\ion{O}{1}]}~$\lambda6363$  & 6365.535  & 1.0     \\
% {[\ion{S}{3}]}~$\lambda9532$  & 9533.2    & 2.4686  \\
% {[\ion{S}{3}]}~$\lambda9069$  & 9071.1    & 1.0     \\
% {[\ion{Ar}{3}]}~$\lambda7135$ & 7137.77   & 4.16988 \\
% {[\ion{Ar}{3}]}~$\lambda7751$ & 7753.19   & 1.0 \\
% {\ion{Mg}{2}}~$\lambda2800a$  & 2796.352  & 1.0     \\
% {\ion{Mg}{2}}~$\lambda2800b$  & 2803.530  & 1.0     \\
\enddata
\tablecomments{Rest-frame vacuum wavelengths and flux ratios for all hydrogen
  and helium recombination lines included in the basis templates relative to H$\beta=1.0$.
%  For forbidden lines, the Relative Flux column gives the flux ratio
%  within each doublet. We sample the overall strength of
%  [\ion{O}{3}]~$\lambda5007$, [\ion{O}{2}],
%  [\ion{N}{2}]~$\lambda6584$, and [\ion{S}{2}]~$\lambda6716$ relative
%  to H$\beta$ from the Gaussian mixture model described
%  in \S\ref{appendix:sps}; we instead fix [\ion{O}{1}], [\ion{S}{3}],
%  and [\ion{Ar}{3}] to representative ratios relative to H$\beta$
%  (\S\ref{appendix:sps}).
}
\end{deluxetable}

